Faster Deterministic Algorithms for Packing, Matching and $t$-Dominating Set Problems

In this paper, we devise three deterministic algorithms for solving the $m$-set $k$-packing, $m$-dimensional $k$-matching, and $t$-dominating set problems in time $O^*(5.44^{mk})$, $O^*(5.44^{(m-1)k})$ and $O^*(5.44^{t})$, respectively. Although recently there has been remarkable progress on randomized solutions to those problems, our bounds make good improvements on the best known bounds for deterministic solutions to those problems.

==> mac90.tex <==
%standard macros for typesetting articles
\hyphenation{super-terse mea-sure semi-recursive non-recursive
             non-superterse}
\newcounter{savenumi}
\newenvironment{savenumerate}{\begin{enumerate}
\setcounter{enumi}{\value{savenumi}}}{\end{enumerate}
\setcounter{savenumi}{\value{enumi}}}
\newtheorem{theoremfoo}{Theorem}%[section] %by chapter in report style
\newenvironment{theorem}{\pagebreak[1]\begin{theoremfoo}}{\end{theoremfoo}}
\newenvironment{repeatedtheorem}[1]{\vskip 6pt
\noindent
{\bf Theorem #1}\ \em
}{}
%\newtheorem{repeatedtheorem}{Theorem} % number this yourself using
%                                      % \def\therepeatedtheorem{text}
%\newtheorem{observationfoo}[theoremfoo]{Observation}
%\newenvironment{observation}{\pagebreak[1]\begin{observationfoo}}{\end{observationfoo}}
\newtheorem{propositionfoo}[theoremfoo]{Proposition}
\newenvironment{proposition}{\pagebreak[1]\begin{propositionfoo}}{\end{propositionfoo}}
%\newtheorem{conventionfoo}[theoremfoo]{Convention}
%\newenvironment{convention}{\pagebreak[1]\begin{conventionfoo}}{\end{conventionfoo}}
\newtheorem{lemmafoo}[theoremfoo]{Lemma}
\newenvironment{lemma}{\pagebreak[1]\begin{lemmafoo}}{\end{lemmafoo}}
\newtheorem{conjecturefoo}[theoremfoo]{Conjecture}
\newenvironment{conjecture}{\pagebreak[1]\begin{conjecturefoo}}{\end{conjecturefoo}}
\newtheorem{corollaryfoo}[theoremfoo]{Corollary}
\newenvironment{corollary}{\pagebreak[1]\begin{corollaryfoo}}{\end{corollaryfoo}}
\newtheorem{exercisefoo}{Exercise}
\newenvironment{exercise}{\pagebreak[1]\begin{exercisefoo}\rm}{\end{exercisefoo}}
%\newtheorem{problemfoo}{Problem}
%\newenvironment{problem}{\pagebreak[1]\begin{problemfoo}\rm}{\end{problemfoo}}
\newtheorem{openfoo}[theoremfoo]{Question}
\newenvironment{open}{\pagebreak[1]\begin{openfoo}}{\end{openfoo}}
\newtheorem{nttn}[theoremfoo]{Notation}
\newenvironment{notation}{\pagebreak[1]\begin{nttn}\rm}{\end{nttn}}

\newtheorem{dfntn}[theoremfoo]{Definition}
\newenvironment{definition}{\pagebreak[1]\begin{dfntn}\rm}{\end{dfntn}}

%\newtheorem{remarkfoo}[theoremfoo]{Remark}
%\newenvironment{remark}{\pagebreak[1]\begin{remarkfoo}}{\end{remarkfoo}}
\newenvironment{proof}
    {\pagebreak[1]{\narrower\noindent {\bf Proof:\quad\nopagebreak}}}{\QED}
%\newenvironment{alternateproof}
%               {{\narrower\noindent {\bf Alternate proof:\quad}}}{\QED}
%\newenvironment{sketch}
%    {\pagebreak[1]{\narrower\noindent {\bf Proof sketch:\quad\nopagebreak}}}{}
\newenvironment{sketch}
    {\pagebreak[1]{\narrower\noindent {\bf Proof sketch:\quad\nopagebreak}}}{\QED}
%\newenvironment{construction}{{\narrower}}{}
%\newenvironment{comment}{$\{$}{$\}$}
\newenvironment{comment}{\penalty -50 $(*$\nolinebreak\ }{\nolinebreak $*)$\linebreak[1]\ }
\renewcommand{\theenumi}{\roman{enumi}}
 % number subtheorems i., ii., iii., iv.,...
\newcommand{\yyskip}{\penalty-50\vskip 5pt plus 3pt minus 2pt}
\newcommand{\blackslug}{\hbox{\hskip 1pt
        \vrule width 4pt height 8pt depth 1.5pt\hskip 1pt}}
%\newcommand{\clearslug}{$\Box$}
%\newcommand{\QEDcomment}[1]{{\penalty10000\parindent 0pt\penalty10000
%        \hskip 8 pt\nolinebreak\blackslug\ #1\hfill\lower 8.5pt\null}
%        \par\yyskip\pagebreak[1]}
%\newcommand{\QEDcomment}[1]{{\penalty10000\parindent 0pt\penalty10000
%        \hskip 8 pt\nolinebreak$\Box$\ #1\hfill\lower 8.5pt\null}
%        \par\yyskip\pagebreak[1]}
%\newcommand{\QED}{\QEDcomment{}}
%\newcommand{\QEDsketch}{{\parindent 0pt\penalty 10000
%       \hskip 8 pt\penalty 10000\clearslug\hfill\lower 8.5pt\null}
%       \par\yyskip}
     
\newcommand{\dash}{{\rm\mbox{-}}}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceiling}[1]{\left\lceil#1\right\rceil}
%\newcommand{\xvec}{x_1,\ldots,x_n}
\newcommand{\st}{\mathrel{:}}
%\newcommand{\domain}{{\em domain}}
%\newcommand{\bit}{{\rm bit}}
%\newcommand{\odd}{{\rm odd}}
%\def\<#1>{\langle#1\rangle}
\newcommand{\ang}[1]{\langle#1\rangle}
\newcommand{\DTIME}{{\rm DTIME}}
%\newcommand{\UTIME}{{\rm UTIME}}
%\newcommand{\RTIME}{{\rm RTIME}}
\newcommand{\DSPACE}{{\rm DSPACE}}
\newcommand{\NSPACE}{{\rm NSPACE}}
\newcommand{\polylog}{\mathop{\rm polylog}}
%\newcommand{\SPARSE}{{\rm SPARSE}}
%\newcommand{\TALLY}{{\rm TALLY}}
\newcommand{\UP}{{\rm UP}}
%\newcommand{\US}{{\rm US}}
\newcommand{\PH}{{\rm PH}}
\newcommand{\R}{{\rm R}}
\newcommand{\NTIME}{{\rm NTIME}}
\newcommand{\PTIME}{{\rm PrTIME}}
%\newcommand{\coNTIME}{{\rm coNTIME}}
%\newcommand{\EXPTIME}{{\rm EXPTIME}}
%\newcommand{\NEXPTIME}{{\rm NEXPTIME}}
%\newcommand{\EXPPTIME}{{\rm EXPPTIME}}
%\newcommand{\NEXPPTIME}{{\rm NEXPPTIME}}
%\newcommand{\DSPACE}{{\rm DSPACE}}
%\newcommand{\NSPACE}{{\rm NSPACE}}
%\newcommand{\LOGSPACE}{{\rm LOGSPACE}}
\newcommand{\PSPACE}{{\rm PSPACE}}
%\newcommand{\RP}{{\rm RP}}
%\newcommand{\PH}{{\rm PH}}
\newcommand{\NE}{{\rm NE}}
\newcommand{\poly}{{\rm poly}}
%\newcommand{\NLOGTIME}{{\rm NLOGTIME}}
%\newcommand{\LOGTIME}{{\rm LOGTIME}}
\newcommand{\LOGSPACE}{{\rm LOGSPACE}}
%\renewcommand{\star}{{\textstyle *}} % used to be 5-pointed star
%\newcommand{\RUNS}{{\rm RUNS}}
%\newcommand{\ESPACE}{{\rm ESPACE}}
%\newcommand{\logtime}{{\rm logtime}}
\newcommand{\E}{{\rm E}}
%\newcommand{\EX}{{\rm EX}}
%\newcommand{\tow}{{\rm tow}}
\newcommand{\SAT}{{\rm SAT}}
%\newcommand{\UniqueSAT}{{\rm UniqueSAT}}
%\newcommand{\LONG}{{\rm LONG}}
%\newcommand{\LMSAT}{{\rm LMSAT}}
%\newcommand{\coNLOGTIME}{\mbox{\rm co-{\rm NLOGTIME}}}
\newcommand{\NP}{{\rm NP}}
\let\paragraphsym\P
\renewcommand{\P}{{\rm P}}      % used to be paragraph sign
\newcommand{\coNP}{{\co\NP}}
%\newcommand{\coUP}{{\co\UP}}
%\newcommand{\N}{{\sf N}}
%\newcommand{\REC}{{\rm REC}}
%\newcommand{\Q}{{\rm Q}}
%\newcommand{\FQ}{{\rm FQ}}
%\newcommand{\MQ}{{\rm MQ}}
%\newcommand{\NQ}{{\rm NQ}}
%\newcommand{\Qp}{\Q_\|}
%\newcommand{\FQp}{\FQ_\|}
%\newcommand{\MQp}{\MQ_\|}
%\newcommand{\BFQ}{{\bf Q}}
%\newcommand{\BFQp}{\BFQ_\|}
%\newcommand{\F}{{\rm F}}
%\renewcommand{\H}{{\rm H}}      % used to be slanted " accent
%\newcommand{\GEQ}{{\rm GEQ}}
%\newcommand{\parity}{{\rm PARITY}}
%\newcommand{\DIF}{{\rm D}}
\newcommand{\propersubset}{\subset}
%\newcommand{\mod}{\mathrel{\rm mod}}
%\renewcommand{\div}{\mathrel{\rm div}} % used to be division sign
%\newcommand{\DIV}{\mathrel{\rm DIV}}
\newcommand{\xor}{\oplus}
\newcommand{\m}{{\rm m}}
\newcommand{\T}{{\rm T}}
\let\savett\tt
\renewcommand{\tt}{{\rm tt}}    % used to be typewriter type style
%\newcommand{\postt}{{\rm ptt}}
%\newcommand{\wtt}{{\rm wtt}}
%\newcommand{\wbtt}{{\rm wbtt}}
\newcommand{\btt}{{\rm btt}}
%\newcommand{\nwtt}{{n\rm\mbox{-}wtt}}
\newcommand{\ntt}{{n\rm\mbox{-}tt}}
\newcommand{\ktt}{{k\rm\mbox{-}tt}}
\newcommand{\kT}{{k\rm\mbox{-}T}}
%\newcommand{\onequery}{{1\rm\mbox{-}T}}
%\newcommand{\nquery}{{n\rm\mbox{-}T}}
%\newcommand{\npquery}{{n\rm\mbox{-}wtt}}
\newcommand{\onett}{{1\rm\mbox{-}tt}}
%\newcommand{\TLE}{\le_\T}
%\newcommand{\TEQV}{\equiv_\T}
%\newcommand{\lognplusone}{\ceiling{\log{(n+1)}}}
%\newcommand{\D}{{\rm D}}
%\newcommand{\Dbar}{\bar{\D}}
\newcommand{\Abar}{{\bar{A}}}
\newcommand{\Bbar}{{\bar{B}}}
\newcommand{\Cbar}{{\bar{C}}}
%\newcommand{\Kbar}{{\bar{K}}}
%\newcommand{\BFD}{{\bf D}}
%\newcommand{\BFnabla}{{\mbox{\boldmath $\nabla$}}}
%\newcommand{\bfn}{{\bf n}}
%\newcommand{\bfnplusone}{{\bf(n+1)}}
%\newcommand{\bfb}{{\bf b}}
%\newcommand{\bfK}{{\bf K}}
%\newcommand{\bfa}{\mbox{\boldmath $a$}}
%\newcommand{\cat}{\mathop{\|}}
%\newcommand{\jump}{^\prime}
%\newcommand{\recursive}{\FQ(0,\emptyset)}
%\newcommand{\Qrecursive}{\Q(0,\emptyset)}
%\newcommand{\frec}{{\rm FREC}}
%\newcommand{\qrec}{{\rm SREC}}
%\newcommand{\bits}{{\{0,1\}}}
%\newcommand{\Xhat}{\widehat{X}}
\def\nre.{$n$\/-r.e.}
%\def\nlr.{$n$\/-l.r.}
%\def\alr.{$a$\/-l.r.}
%\def\blr.{$b$\/-l.r.}
%\def\lr.{l.r.}
%\def\re.{r.e.}
%\newcommand{\card}{{\rm card}}
%\newcommand{\bffunction}{\mbox{\bf function}}
%\newcommand{\bfvar}{\mbox{\bf var}}
%\newcommand{\bfbegin}{\mbox{\bf begin}}
%\newcommand{\bffor}{\mbox{\bf for}}
%\newcommand{\bfto}{\mbox{\bf to}}
%\newcommand{\bfdo}{\mbox{\bf do}}
%\newcommand{\bfwhile}{\mbox{\bf while}}
%\newcommand{\bfnot}{\mbox{\bf not}}
%\newcommand{\bfif}{\mbox{\bf if}}
%\newcommand{\bfthen}{\mbox{\bf then}}
%\newcommand{\bfend}{\mbox{\bf end}}
%\newcommand{\bfreturn}{\mbox{\bf return}}
%\newcommand{\bfand}{\mbox{\bf and}}
%\newcommand{\bfprogram}{\mbox{\bf program}}
%\newcommand{\bfmachine}{\mbox{\bf machine}}
%\newcommand{\bfelse}{\mbox{\bf else}}
%\newcommand{\bfsimulate}{\mbox{\bf simulate}}
%\newcommand{\bfrepeat}{\mbox{\bf repeat}}
%\newcommand{\bfuntil}{\mbox{\bf until}}
%\newcommand{\TC}{{\cal T}}
%\newcommand{\QC}{{\cal Q}}
%\newcommand{\FP}{{\rm FP}}
%\newcommand{\DTWOP}{\Delta_2^\P}
%\newcommand{\cvg}{\!\downarrow\,}
%\newcommand{\dvg}{\!\uparrow\,}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}
\newenvironment{multi}{\left\{\begin{array}{ll}}{\end{array}\right.}
\newcommand{\union}{\cup}
\newcommand{\Union}{\bigcup}
\newcommand{\intersection}{\cap}
\newcommand{\Intersection}{\bigcap}
%\newcommand{\implies}{\Rightarrow}
%\newcommand{\ifff}{$\Leftrightarrow$\ }
%\newcommand{\vect}[1]{\vec{#1}\/}
\newcommand{\OR}{\vee}
\newcommand{\AND}{\wedge}
\newcommand{\reason}[1]{\mbox{\qquad\rm #1}}     % added quad 8/9, qquad 8/31
\newcommand{\nlreason}[1]{\\ & & \mbox{\rm #1}}  % killed comma 8/31
%\newcommand{\ddx}{{d \over {dx}}}
\newcommand{\infinity}{\infty}
%\newcommand{\logsum}{\hbox{\rm logsum}}
%\newcommand{\logprod}{\hbox{\rm logprod}}
%\newcommand{\integral}{\int}
%\newcommand{\chir}{\chi^{\rm r}}
%\newcommand{\dx}{\,dx}
%\newcommand{\RANGE}{{\rm RANGE}}
%\newcommand{\EVENBET}{{\rm EVENBET}}
%\newcommand{\BETTINGPOOL}{{\rm BETTINGPOOL}}
%\newcommand{\e}{\{e\}}
%\newcommand{\INF}{{\rm INF}}
%\newcommand{\TOT}{{\rm TOT}}
%\newcommand{\join}{\vee}
%\newcommand{\join}{\mathrel{\rm join}}
\newcommand{\implies}{\mathrel{\Rightarrow}}
\newcommand{\Implies}{\mathrel{\Longrightarrow}}
%\newcommand{\ifandonlyif}{\mathrel{\Leftrightarrow}}
\newcommand{\Iff}{\mathrel{\Longleftrightarrow}}
%\newcommand{\del}{\mathop{\nabla}}
\newcommand{\scrod}{\quad\nopagebreak}
%\newcommand{\ldotss}{\ldots {}}
%\newcommand{\support}{This research was supported in part
%by grant number CCR-8808949 from the National Science
%Foundation.}
%\newcommand{\Kleenestar}{{\textstyle *}}
\newcommand{\ACCEPT}{{\rm ACCEPT}}
\newcommand{\PARITY}{{\rm PARITY}}
%\newcommand{\PARITYP}{\PARITY\dash\P}
\newcommand{\PARITYP}{\PARITY\P}
\newcommand{\MOD}{{\rm MOD}}
%\newcommand{\MODkP}{\MOD_k\P}
%\newcommand{\MODjP}{\MOD_j\P}
\newcommand{\PP}{{\rm PP}}
%\newcommand{\TP}{{\rm TP}}
\newcommand{\FewP}{{\rm FewP}}
\newcommand{\EP}{{\rm EP}}
\tolerance=2000
\def\pmod#1{\allowbreak\mkern6mu({\rm mod}\,\,#1)}
\newcommand{\co}{{\rm co}\dash}
\newcommand{\PF}{{\rm PF}}
\newcommand{\EXP}{{\rm EXP}}
\newcommand{\NEXP}{{\rm NEXP}}
\newcommand{\Hastad}{H{\aa}stad}
\newcommand{\Kobler}{K\"obler}
\newcommand{\Schoning}{Sch\"oning}
\newcommand{\Toran}{Tor\'an}
\newcommand{\Balcazar}{Balc{\'a}zar}
\newcommand{\Diaz}{D\'{\i}az}
\newcommand{\Gabarro}{Gabarr{\'o}}
\newcommand{\RIA}{CCR-8808949}
\newcommand{\PYI}{CCR-8958528}
\newcommand{\NSFFT}{CCR-9415410}
\newcommand{\NSFALEXIS}{CCR-9522084}
\newtheorem{factfoo}[theoremfoo]{Fact}
\newenvironment{fact}{\pagebreak[1]\begin{factfoo}}{\end{factfoo}}
\newenvironment{acknowledgments}{\par\vskip 20pt\noindent{\footnotesize\em Acknowledgments.}\footnotesize}{\par}
%\newcommand{\pbtt}{{\rm pbtt}}
%\newcommand{\UnSAT}{{\rm UnSAT}}
%\newcommand{\bpp}{{\rm bpp}}
%\newtheorem{xmpl}[theoremfoo]{Example}
%\newenvironment{example}{\pagebreak[1]\begin{xmpl}\rm}{\end{xmpl}}
%\newcommand{\Boole}{{\rm Bf}}
%\newcommand{\pT}{{\rm pT}}
\newcommand{\POLYLOGSPACE}{{\rm POLYLOGSPACE}}
\newcommand{\SPACE}{{\rm SPACE}}
%\newcommand{\logspace}{{\rm logspace}}
\newcommand{\BPP}{{\rm BPP}}
%\newcommand{\extend}{\supset}
%\newcommand{\onewtt}{{1\dash\wtt}}
\newcommand{\lookatme}{\marginpar[$\Rightarrow$]{$\Leftarrow$}}
\newcommand{\muchless}{\ll}
\newcommand{\plusminus}{\pm}
\newcommand{\nopagenumbers}{\renewcommand{\thepage}{\null}}
\newenvironment{algorithm}{\renewcommand{\theenumii}{\arabic{enumii}}\renewcommand{\labelenumii}{Step \theenumii :}\begin{enumerate}}{\end{enumerate}}
\newcommand{\squeeze}{
\textwidth 6in
\textheight 8.8in
\oddsidemargin 0.2in
\topmargin -0.4in
}
\newcommand{\existsunique}{\exists \! ! \,}
\newcommand{\YaleAddress}{Yale University,
Dept.\ of Computer Science,
P.O.\ Box 208285, Yale Station,
New Haven, CT\ \ 06520-8285.
Email: {\savett beigel-richard@cs.yale.edu}}
\newcommand{\pageline}[2]{[{\bf p.~#1, l.~#2}]}
\newcommand{\Beigel}{Richard Beigel\thanks{\newsupport} \\
Yale University \\
Dept.\ of Computer Science \\
P.O. Box 208285, Yale Station \\
New Haven, CT\ \ 06520-8285}

\newcommand{\newsupport}{Supported in part by grants \RIA\ and \PYI\
from the National Science Foundation}
\newtheorem{propertyfoo}[theoremfoo]{Property}
\newenvironment{property}{\pagebreak[1]\begin{propertyfoo}}{\end{propertyfoo}}


\makeatletter

\def\@makechapterhead#1{ \vspace*{50pt} { \parindent 0pt \raggedright 
 \ifnum \c@secnumdepth >\m@ne \huge\bf \@chapapp{} \thechapter. \par 
 \vskip 20pt \fi \Huge \bf #1\par 
 \nobreak \vskip 40pt } }

\def\@sect#1#2#3#4#5#6[#7]#8{\ifnum #2>\c@secnumdepth
     \def\@svsec{}\else 
     \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname.\hskip 1em }\fi
     \@tempskipa #5\relax
      \ifdim \@tempskipa>\z@ 
        \begingroup #6\relax
          \@hangfrom{\hskip #3\relax\@svsec}{\interlinepenalty \@M #8\par}
        \endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                      \protect\numberline{\csname the#1\endcsname}\fi
                    #7}\else
        \def\@svsechd{#6\hskip #3\@svsec #8\csname #1mark\endcsname
                      {#7}\addcontentsline
                           {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                             \protect\numberline{\csname the#1\endcsname}\fi
                       #7}}\fi
     \@xsect{#5}}

\def\@begintheorem#1#2{\it \trivlist \item[\hskip \labelsep{\bf #1\ #2.}]}

\def\@opargbegintheorem#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3).}]}

\makeatother

%%Clean up section headers.  Period after section number.  Smaller font.
%\makeatletter
%\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus -1ex minus 
% -.2ex}{2.3ex plus .2ex}{\large\bf}}
%\makeatother
%\def\thesection {\arabic{section}.}
%\def\thesubsection {\thesection\arabic{subsection}.}
%\def\thesubsubsection {\thesubsection\arabic{subsubsection}.}
%\def\theparagraph {\thesubsubsection\arabic{paragraph}.}
%\def\thesubparagraph {\theparagraph\arabic{subparagraph}.}

\newcommand{\kstar}{{\textstyle *}}
\newcommand{\F}[2]{F_{#1}^{#2}}
\newcommand{\FQ}[2]{\PF_{{#1\rm\mbox{-}T}}^{#2}}
\newcommand{\Q}[2]{\P_{{#1\rm\mbox{-}T}}^{#2}}
\newcommand{\FQp}[2]{\PF_{{#1\rm\mbox{-}tt}}^{#2}}
\newcommand{\Qp}[2]{\P_{{#1\rm\mbox{-}tt}}^{#2}}
\newcommand{\ppoly}{\P/\poly}
\newcommand{\pnplog}{\P^{\NP[\log]}}
\newcommand{\pleq}[1]{\leq_{#1}^{p}}

\def\abs#1{\left|#1\right|}
\def\exp#1{{\rm exp}\left(#1\right)}
\newcommand{\transfig}[1]{\begin{center}\vspace{-6pt}\input{#1.tex}\vspace{-12pt}\end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% Bibliography Stuff %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% By Richard Beigel and Nick Reingold %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifshortconferences
\shortconferencesfalse
\newif\ifmediumconferences
\mediumconferencesfalse

\def\ending#1{{\count1=#1\relax
% mod out by 100 first
\count2=\count1
\divide\count2 by 100
\multiply\count2 by 100
\advance\count1 by -\count2
%
\ifnum\count1=11
th%
\else \ifnum\count1=12
th%
\else \ifnum\count1=13
th%
\else 
\count2=\count1
\divide\count1 by 10
\multiply\count1 by 10
\advance\count2 by -\count1
\ifnum\count2=1
st%
\else \ifnum\count2=2
nd%
\else \ifnum\count2=3
rd%
\else th%
\fi\fi\fi\fi\fi\fi
}}

\def\STOC{\conf{STOC}}
\def\STOCname{\ifshortconferences ACM STOC\else\ifmediumconferences Ann. ACM Symp. Theor. Comput.\else Annual ACM Symposium on Theory of Computing\fi\fi}
\def\STOCzero{68}

\def\FOCS{\conf{FOCS}}
\def\FOCSname{\ifshortconferences IEEE FOCS\else\ifmediumconferences Ann. Symp. Found. Comput. Sci.\else IEEE Symposium on Foundations of Computer Science\fi\fi}
\def\FOCSzero{59}

\def\FSTTCS{\conf{FSTTCS}}
\def\FSTTCSname{\ifshortconferences FST\&TCS\else\ifmediumconferences Ann. Conf. Found. Softw. Theor. and Theor. Comp. Sci.\else Conference on Foundations of Software Theory and Theoretical Computer Science\fi\fi}
\def\FSTTCSzero{80}

\def\Complexity{\conf{Complexity}}
\def\Complexityname{\ifshortconferences Conf. Computational Complexity\else\ifmediumconferences Ann. Conf. Computational Complexity\else Annual Conference on Computational Complexity\fi\fi}
\def\Complexityzero{85}
\def\ComplexityOne{Structure in Complexity Theory}

\def\Structures{\conf{Structures}}
\def\Structuresname{\ifshortconferences Ann. Conf. Structure in Complexity Theory\else\ifmediumconferences Ann. Conf. Structure in Complexity Theory\else Annual Conference on Structure in Complexity Theory\fi\fi}
\def\Structureszero{85}
\def\StructuresOne{Structure in Complexity Theory}

\def\SODA{\conf{SODA}}
\def\SODAname{\ifshortconferences ACM-SIAM Symp. on Discrete Algorithms\else Annual ACM-SIAM Symposium on Discrete Algorithms\fi}
\def\SODAzero{89}

\def\STACS{\conf{STACS}}
\def\STACSname{\ifshortconferences STACS\else\ifmediumconferences\else Annual Symposium on Theoretical Aspects of Computer Science\fi\fi}
\def\STACSzero{83}

\def\SPAA{\conf{SPAA}}
\def\SPAAname{\ifshortconferences ACM SPAA\else\ifmediumconferences Ann. ACM Symp. Par. Alg. Arch.\else Annual ACM Symposium on Parallel Algorithms and Architectures\fi\fi}
\def\SPAAzero{88}

\def\Proceedings{\ifshortconferences Proc.\else\ifmediumconferences Proc.\else Proceedings\fi\fi}
\def\Proceedingsofthe{\ifshortconferences Proc.\else\ifmediumconferences Proc.\else Proceedings of the\fi\fi}

\newcounter{confnum}

\def\conf#1#2{%
\setcounter{confnum}{#2}%
\addtocounter{confnum}{-\csname #1zero\endcsname}%
\ifnum\value{confnum}=1%
\expandafter\ifx\csname #1One\endcsname\relax%
\Proceedingsofthe\ \arabic{confnum}\ending{\value{confnum}}\ \csname #1name\endcsname%
\else \csname #1One\endcsname\fi%
\else%
\Proceedingsofthe\
\arabic{confnum}\ending{\value{confnum}}\ \csname #1name\endcsname\fi}

%%%%%%%%%%%%   end bibliography stuff   %%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% QED/LABELS %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% \qed       Inserts a QED symbol (\qsym) at the end
%%            of the line, unless there is not enough
%%            room, in which case the QED symbol goes
%%            at the end of the next line.
%% 
%% \noqed     Supresses the very next invocation of \qed.
%% 
%% \eqnqed    Inside an eqnarray*, this puts a QED
%%            symbol at the (right) end of the current
%%            line.  It also supresses the next
%%            invocation of \qed.
%% 
%% \eqnlabel  Inside an eqnarray*, this makes a
%%            user-defined equation label.  The macro
%%            takes two args.  The first is displayed
%%            as the equation ``number.''  The second
%%            is the internal LaTeX reference key.
%%            Thus the call \eqnlabel{foo}{bar}
%%            creates an equation (foo) which you can
%%            refer to with \ref{bar} and
%%            \pageref{bar}.
%% 
%% Both \eqnqed and \eqnlabel should be placed just before \\
%% or \end{eqnarray*}.  If \eqnlabel is used on a line which is
%% not the last line of the eqnarray,  the \\ is still
%% required.
%%
%% Both \eqnqed and \eqnlabel may be used in eqnarray or
%% equation environments without disturbing the usual
%% numbering system.  (Any number which would have been used
%% is used for the next equation.)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% Put your favorite QED symbol here.			   
%%
\def\qsym{\vrule width0.7ex height0.9em depth0ex}


%%
%% A switch to turn the symbol on or off.  Normally it is on.
%%
\newif\ifqed\qedtrue


%%
%% The next invocation of \qed in suppressed with this
%% command.
%% 
\def\noqed{\global\qedfalse}


%%
%% This definition is (essentially) from the TeXbook.
%%
\def\qed{\ifqed{\penalty1000\unskip\nobreak\hfil\penalty50
\hskip2em\hbox{}\nobreak\hfil\qsym
\parfillskip=0pt \finalhyphendemerits=0\par\medskip}\fi\global\qedtrue}

\def\QEDcomment#1{\ifqed{\penalty1000\unskip\nobreak\hfil\penalty50
\hskip2em\hbox{}\nobreak\hfil\qsym\ #1
\parfillskip=0pt \finalhyphendemerits=0\par\medskip}\fi\global\qedtrue}

%%
%% The eqnqed/label hack is accomplished by mucking
%% around with some internal LaTeX definitions.  
%%
\makeatletter
\def\eqnqed{\noqed
	\def\@tempa{equation}
	\ifx\@tempa\@currenvir\def\@eqnnum{\qsym}%
	\addtocounter{equation}{-1}\else%
%    \def\theequation{{\qsym}}% [not needed]
    \def\@@eqncr{\let\@tempa\relax
    \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}%
      \else \def\@tempa{&}\fi
     \@tempa {\def\@eqnnum{{\qsym}}\@eqnnum}%  [changed theequation to @eqnnum]
     \global\@eqnswtrue\global\@eqcnt\z@\cr}\fi}

%% OLD VERSION
%% 
%% \def\eqnqed{\noqed\@eqnswtrue%
%%     \def\@@eqncr{\let\@tempa\relax
%%     \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}%
%%       \else \def\@tempa{&}\fi
%%      \@tempa \qsym%
%%      \global\@eqnswtrue\global\@eqcnt\z@\cr}}
%% 

%%
%% The same trick can be used to produce arbitrary labels for
%% equations.
%%
\def\eqnlabel#1#2{\if@filesw {\let\thepage\relax%
   \def\protect{\noexpand\noexpand\noexpand}%
   \edef\@tempa{\write\@auxout{\string
      \newlabel{#2}{{{#1}}{\thepage}}}}%
   \expandafter}\@tempa%
   \if@nobreak \ifvmode\nobreak\fi\fi\fi%
	\def\@tempa{equation}
	\ifx\@tempa\@currenvir\def\theequation{{#1}}% 
	\addtocounter{equation}{-1}\else%
%    \def\theequation{{#1}}% [not needed]
    \def\@@eqncr{\let\@tempa\relax
    \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}%
      \else \def\@tempa{&}\fi
     \@tempa {\def\@eqnnum{{#1}}\@eqnnum}% [changed theequation to @eqnnum]
     \global\@eqnswtrue\global\@eqcnt\z@\cr}\fi}



\makeatother

%% end of qed/eqnlabel

\newcommand{\listqed}{\qed\noqed} % RJB - use if proof ends with a list
% RJB Use \littleqed at the end of proving assertions inside proofs
\def\littleqed{\ifqed{\penalty1000\unskip\nobreak\hfil\penalty50
\hskip2em\hbox{}\nobreak\hfil\littleqsym
\parfillskip=0pt \finalhyphendemerits=0\par\medskip}\fi\global\qedtrue}
\def\littleqsym{\vrule width0.6ex height0.6em depth0ex}
\def\QED{\qed}

\makeatother

%% end of qed/eqnlabel
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   end of Nick's qed stuff   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\aftereqnskip{\vskip-3pt} % compositor, please adjust this

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SPASAM}[1]{{\rm MOL\dash A}(#1)}
\newcommand{\SPASM}[1]{{\rm MOL'}(#1)}
\newcommand{\SPAM}[1]{{\rm MOL}(#1)}
\newcommand{\NPbits}[1]{{\rm NPbits}(#1)}
\newcommand{\NPinit}[1]{{\rm NPinit}(#1)}
\newcommand{\NPpaths}[1]{{\rm NPpaths}(#1)}
\newcommand{\LOR}{\bigvee}

\newcommand{\set}[1]{\left\{{#1}\right\}}


